Actor-Critic Network for O-RAN Resource Allocation: xApp Design, Deployment, and Analysis

Open Radio Access Network (O-RAN) has introduced an emerging RAN architecture that enables openness, intelligence, and automated control. The RAN Intelligent Controller (RIC) provides the platform to design and deploy RAN controllers. xApps are the applications which will take this responsibility by leveraging machine learning (ML) algorithms and acting in near-real time. Despite the opportunities provided by this new architecture, the progress of practical artificial intelligence (AI)-based solutions for network control and automation has been slow. This is mostly because of the lack of an endto-end solution for designing, deploying, and testing AI-based xApps fully executable in real O-RAN network. In this paper we introduce an end-to-end O-RAN design and evaluation procedure and provide a detailed discussion of developing a Reinforcement Learning (RL) based xApp by using two different RL approaches and considering the latest released O-RAN architecture and interfaces.

==> include/Parameters.tex <==

\begin{table}[ht]
\centering
\caption{Testing Parameters.}
%\resizebox{0.85\textwidth}{!}{%
%\begin{tabular}{|c|c|c|c|}
{\begin{tabular}{|p{4.0cm}|p{1.4cm}|}
\hline
\vspace{0.02 in}
\textbf{Network Parameters} & \vspace{0.02 in}\textbf{Value} \\
\vspace{0.02 in} \\ \hline
%\vspace{0.001 in}
Number of Hidden Layers &
%\vspace{-0.05 in}
4

%\vspace{-0.1 in}
\\ \hline
Number of Neurons &
%\vspace{-0.05 in}
384
%\vspace{-0.1 in}

%\vspace{-0.1 in}
\\ \hline
%\vspace{0.001 in}
Number of gNB &
%\vspace{-0.05 in}
5
%\vspace{-0.1 in}

%\vspace{-0.1 in}
\\ \hline
%\vspace{0.001 in}
No. of Channels per gNB &
%\vspace{-0.05 in}
2
%\vspace{-0.1 in}

%\vspace{-0.1 in}
\\ \hline
%\vspace{0.001 in}
Number of Ues &
%\vspace{-0.05 in}
12
%\vspace{-0.1 in}

%\vspace{-0.1 in}
\\ \hline
%\vspace{0.001 in}
Maximum Traffic load per UE(Downlink)r &
%\vspace{-0.05 in}
2 Mbps
%\vspace{-0.1 in}

%\vspace{-0.1 in}
\\ \hline
%\vspace{0.001 in}
Frequency  &
%\vspace{-0.05 in}
6 GHz
%\vspace{-0.1 in}

%\vspace{-0.1 in}
\\ \hline
%\vspace{0.001 in}
Bandwidth &
%\vspace{-0.05 in}
10 MHz
%\vspace{-0.1 in}

%\vspace{-0.1 in}
\\ \hline

%\vspace{0.001 in}
Tx &
%\vspace{-0.05 in}
20 dBm
%\vspace{-0.1 in}

%\vspace{-0.1 in}
\\ \hline

%\vspace{0.001 in}
Discount factor &
%\vspace{-0.05 in}
0.99
%\vspace{-0.1 in}

%\vspace{-0.1 in}
\\ \hline

%\vspace{0.001 in}
Actor learning-rate &
%\vspace{-0.05 in}
0.01
%\vspace{-0.1 in}

%\vspace{-0.1 in}
\\ \hline

%\vspace{0.001 in}
Critic learning-rate &
%\vspace{-0.05 in}
0.04
%\vspace{-0.1 in}

%\vspace{-0.1 in}
\\ \hline


%\vspace{0.001 in}
Optmizer &
%\vspace{-0.05 in}
Adam
%\vspace{-0.1 in}

%\vspace{-0.1 in}
\\ \hline


%\vspace{0.001 in}
Number of Timeslots per Episode &
%\vspace{-0.05 in}
1000
%\vspace{-0.1 in}

%\vspace{-0.1 in}
\\ \hline

%\vspace{0.001 in}
Number of Episodes &
%\vspace{-0.05 in}
500~700
%\vspace{-0.1 in}

%\vspace{-0.1 in}
\\ \hline
\end{tabular}%
}

\label{tab:xapps}
\end{table}

==> include/xapp_table.tex <==

\begin{table}[ht]
\centering
\caption{Recent xApps provided by the O-RAN Software Community.}
\label{tab:xapp}
%\resizebox{0.85\textwidth}{!}{%
%\begin{tabular}{|c|c|c|c|}
{\begin{tabular}{|p{1.2cm}|p{1.2cm}|p{4.8cm}|}
\hline
\vspace{0.02 in} \textbf{xApp} & \vspace{0.02 in} \textbf{Developer} & \vspace{0.02 in} \textbf{Description} \\ \hline
\vspace{0.05 in}
RC (RAN Control) &
%\vspace{-0.05 in}
\vspace{0.05 in}
Mavenir 
%\vspace{-0.1 in}
&
%\vspace{-0.05 in}
This xApp implements subset of E2 Service Model (SM) RAN Control and enables efficient control of the RAN, including radio bear control, radio access control, and connected mode mobility. 
%\vspace{-0.1 in}
\\ \hline
\vspace{0.03 in}
LP (Load Prediction) &
%\vspace{-0.05 in}
\vspace{0.03 in}
China Mobile 
%\vspace{-0.1 in}
&
%\vspace{-0.05 in}
Developed in python and included a trained ML model for traffic predictions that can be used by another xApp called Traffic Steering (TS).
%\vspace{-0.1 in}
\\ \hline
\vspace{0.02 in}
AD (Anomaly Detection) &
\vspace{0.02 in}
HCL
%\vspace{-0.1 in}
&
%\vspace{-0.05 in}
Developed in Python, it fetches UE data regularly from the SDL, monitors UE metrics,  employs a ML based prediction method to detect anomalous users, and sends the information %related to such user 
to the TS xApp. %to find the anomalous UEs. 
%\vspace{-0.1 in}
\\ \hline
\vspace{0.02 in}
QP (QoE Predictor) &
\vspace{0.02 in}
HCL
%\vspace{-0.1 in}
&
%\vspace{-0.05 in}
Developed in Python, %. This xApp Include prediction for current serving cell. I
it receives a %feature 
set of metrics for a given UE, predicts throughput %predictions 
on the serving and neighbor cells, and sends it to the TS xApp.
%\vspace{-0.1 in}
\\ \hline
\vspace{0.02 in}
Traffic Steering (TS) &
\vspace{0.02 in}
UTFPR (University, Parana, Brazil)
%\vspace{-0.1 in}
&
%\vspace{-0.05 in}
Developed in C++, %programming language. This xApp 
it uses the A1 Policy Intent, listens for poorly performing UEs, sends prediction requests to the QP Driver, and listens for messages that show UE throughput predictions in different cells for making handover decisions. % about UE .
%\vspace{-0.1 in}
\\ \hline
\vspace{0.02 in}
Bouncer &
\vspace{0.02 in}
HCL
%\vspace{-0.1 in}
&
%\vspace{-0.05 in}
Increases performance and functional testing capabilities and %continues 
identifies RIC platform bottlenecks.
%\vspace{-0.1 in}
\\ \hline
\vspace{0.02 in}
KPIMON  &
\vspace{0.02 in}
Samsung
%\vspace{-0.1 in}
&
%\vspace{-0.05 in}
Developed in C and Go, it %. KPIMON xApp is developed to 
collects RAN and system key performance indicators (KPI) from E2 Nodes and write them into the SDL.
%\vspace{-0.1 in}
\\ \hline
\vspace{0.02 in}
NexRAN---Closed-loop RAN slicing &
\vspace{0.02 in}
POWDER, University of Utah
%\vspace{-0.1 in}
&
%\vspace{-0.05 in}
Developed in C++, it provides low-level RAN control, realizing policy driven closed-loop control of RAN slices by getting the current parameters of the RAN elements and controls the slice %behavior 
through the custom slicing service model.
%\vspace{-0.1 in}
\\ \hline
\end{tabular}%
}

\label{tab:xapps}
\end{table}
